Dexterous In-Hand Manipulation of Slender Cylindrical Objects through Deep Reinforcement Learning with Tactile Sensing

Continuous in-hand manipulation is an important physical interaction skill, where tactile sensing provides indispensable contact information to enable dexterous manipulation of small objects. This work proposed a framework for end-to-end policy learning with tactile feedback and sim-to-real transfer, which achieved fine in-hand manipulation that controls the pose of a thin cylindrical object, such as a long stick, to track various continuous trajectories through multiple contacts of three fingertips of a dexterous robot hand with tactile sensor arrays. We estimated the central contact position between the stick and each fingertip from the high-dimensional tactile information and showed that the learned policies achieved effective manipulation performance with the processed tactile feedback. The policies were trained with deep reinforcement learning in simulation and successfully transferred to real-world experiments, using coordinated model calibration and domain randomization. We evaluated the effectiveness of tactile information via comparative studies and validated the sim-to-real performance through real-world experiments.

==> suggested_reviewers.tex <==
Pls put these 4 reviewers in the Tmech web form:

Prof Chenguang Yang
Affiliation: Robot Teleoperation Group, Bristol Robotics Laboratory, University of the West of England Bristol
Email: Charlie.Yang@uwe.ac.uk
Reason: Expert in learning-based manipulation and grasping, robot manipulators, adaptive neural control.
Website: https://people.uwe.ac.uk/Person/CharlieYang

Dr Chengxu Zhou 
Affiliation: University of Leeds
Email: C.X.Zhou@leeds.ac.uk
Reason: Expert in robotic hand design, tele-operation of mobile manipulators, neural network based control.
Website: https://eps.leeds.ac.uk/mechanical-engineering/staff/1720/dr-chengxu-zhou

Prof Nathan Lepora
Affiliation: Dexterous Robotics Group, University of Bristol
Reason: Expert in biomimetics, design and simulation of tactile sensors, learning-based grasping and manipulation with high-resolution tactile feedback.
Website: https://lepora.com/

Dr Lorenzo Jamone
Affiliation: School of Engineering and Materials Science (SEMS) of the Queen Mary University of London
Reason: Expert in robotic manipulation, tactile sensing, robot learning and haptics
Website: https://www.sems.qmul.ac.uk/staff/l.jamone

%%%%%%%%%%% pls also check Tmech new web form see what is needed now


